Holographic neutron stars at finite temperature

We use gauge gravity duality to describe the strange metal phase of High $T_c$ superconductors.

==> Chapters/abbr.tex <==
AI
NN
GPU
CNN
ADC
SPL
DNN
AED
NAS
LTI
DSP
MLP
LSTM
IR
KLT
ROI
LED

==> Chapters/my_publications.tex <==
\chapter*{Publications}
\markboth{Publications}{Publications}
\addcontentsline{toc}{chapter}{Publications}

\vspace*{2em}

\subsection*{Journal publications}

\vspace*{1em}

\begin{enumerate}[wide = 0pt, widest = {[4]}, leftmargin =*]

\item[{[1]}] \textbf{G. Z}, A. A, G. G, G. G, and L.~G. N.
\newblock {Paper Title}.
\newblock \emph{Journal Name}, VOL(NUMBER), PP-PP, YEAR.

\end{enumerate}

\subsection*{Full papers in conference proceedings}
\vspace*{1em}

\begin{enumerate}[wide = 0pt, widest = {[4]}, leftmargin =*]
\item[{[5]}] \textbf{G. Z}, G. W, P. V, H.B. R, M. M, Á. L.
\newblock {Paper Title}.
\newblock In \emph{Proceedings of the Xth Annual International Conference on Conference}, DISTRIBUTOR, PP-PP, YEAR.
\end{enumerate}

\subsection*{Further related publications}
\vspace*{1em}

\begin{enumerate}[wide = 0pt, widest = {[15]}, leftmargin =*]

\item[{[8]}] \textbf{G. Z}, A. B, G. K, G. H, and L.~G. N.
\newblock {Paper Title}.
\newblock In \emph{The Xth Jubilee Conference of Something: Volume of extended abstracts.}, YEAR.

\end{enumerate}

==> Old/chapter_3_-_Copy.tex <==
\chapter{Holographic neutron stars}
\label{holoneutronstars}

This chapter is a review of the paper \cite{2018JHEP...05..118A} where the main equations are presented, this work presents the basic ideas that we will later extend as the cornerstone of our thesis. 

\section{Neutron stars at zero temperature}
The work of \cite{deBoer:2009wk} is the initial point of our main work studying holographic neutron stars. In the above-mentioned paper they solve the TOV equations numerically, in a asymptotically anti-de Sitter space. Just like in the works \cite{toveq,vaganov} their find a maximum value for the mass as a function of the chemical potential at the center, the implications of this have already been explained in section \ref{turningpoint}.  From holographic viewpoint the OV limit in the CFT is associate with the region after the instability but looking the function $M(\epsilon_{F})$ where $\epsilon_{F}$ is the Fermi energy. They assume for the gravity part that beyond the OV limit the star collapses and forms a black hole and for the CFT the fermionic operator $\phi$ starts to mix with generic states and thermalizes. They suggest that the collapse is associated with a phase transition that turns a high density (baryonic) state into a thermal state (quark gluon plasma).\\
In Sections \ref{sec:bulk3} and \ref{sec:correlators3} I will present the main equations that were used in \cite{2018JHEP...05..118A} to describe a holographic neutron star since they are the same equations that we will use for the research carried out in this thesis.

\section{The bulk: self gravitating fermionic fluid at finite temperature}
\label{sec:bulk3}
%
To describe their system they use a very large number of neutral self-gravitating fermions in thermodynamic equilibrium, treated within a $3+1$ asymptotically AdS spacetime. The Einstein equations for such system read
%
\begin{equation}
G_{\mu\nu}+\Lambda g_{\mu\nu}= 8\pi G\, T_{\mu\nu}\,,
\label{eq:einstein-crudas}
\end{equation}
%
being $\Lambda$ a negative cosmological constant, that can be written in terms of the AdS length $L$ as $\Lambda=-3/L^2$, and $G$ the gravitational constant\footnote{Throughout this paper we work in natural units $\hbar=c=k_B=1$.}. Regarding the fermion energy-momentum tensor, we approximate it as a perfect fluid
%
\begin{equation}
T_{\mu\nu}=P g_{\mu\nu}+(\rho+P)u_\mu u_\nu\,.
\label{eq:energy-momentum}
\end{equation}
%
Since we are interested in the limit $mL\gg 1$ in which there is a huge amount of particles within one AdS radius \cite{deBoer:2009wk}, the density and pressure are given by the equations %
\begin{align}
\rho &= \frac{g}{8\pi^3}\int f(p)\sqrt{p^2+m^2 }\,d^3p\,,
\label{eq:rho}\\
P &= \frac{g}{24\pi^3}\int
f(p)\frac{p^2}{\sqrt{p^2+m^2 }} \,d^3p,
\label{eq:p}
\end{align}
%
here $g$ is the number of fermionic species (or the spin degeneracy), the integration runs over all momentum space,
and the function $f(p)$
%
\begin{equation}
f(p)=\frac1{e^{\beta\left(\sqrt{p^2+ m^2}-\mu\right)}+1} \,,
\label{eq:fermi-dirac-distribution}
\end{equation}
%
is the Fermi-Dirac distribution function for a fermion of mass $m$, where $1/\beta=T$ is the local temperature and $\mu$ is the local chemical potential. This expression sets a double parametric dependence of the density $\rho$ and pressure $P$ on the temperature $T$ and chemical potential $\mu$, which in turn depend on the metric as explained below.

As we will deal with equilibrium configurations of neutral fermions in global AdS, we consider an stationary spherically symmetric metric with the form
%
\begin{equation}
ds^2=L^2\left(-e^{\nu(r)}\,dt^2+e^{\lambda(r)}\,dr^2+r^2\,d\Omega^2_2\right)\, ,
\label{eq:metricAdS}
\end{equation}
%
with $d\Omega^2_2=d\vartheta^2+\sin^2{\vartheta}d\varphi^2$. In this setup, the local temperature and chemical potential are  radial functions. They are defined by the thermodynamic equilibrium conditions of Tolman  $e^{\nu(r)/2} T=$constant, and Klein  $e^{\nu(r)/2} \mu=$constant, respectively.

In what follows we find convenient to re-scale the temperature and chemical potential as the dimensionless combinations $\tilde \mu=\mu/m$ and $\tilde T=T/m={1}/{\tilde \beta}$. The Tolman condition is then solved by
%
\begin{equation}
\tilde T=\tilde T_0 e^{\frac{\nu_0-\nu(r)}{2}}\, ,
\label{eq:tolman3}
\end{equation}
%
in terms of the re-scaled temperature $\tilde T_0$ and metric component $\nu_0$ measured at a reference point. The Klein condition can then be rewritten as
%
\begin{equation}
\tilde \mu=\tilde \mu_0 e^{\frac{\nu_0-\nu(r)}{2}}\, ,
\label{eq:klein3}
\end{equation}
%
where $\tilde \mu_0$ is the value of the re-scaled chemical potential at the same reference point.

Further re-scalings of the energy density and pressure as $\tilde \rho=GL^2\rho $ and $\tilde P= GL^2P$ gives the result
%
\begin{align}
\tilde\rho &= \gamma^2\int_1^\infty \frac{\epsilon^2\sqrt{\epsilon^2-1}}{e^{\tilde \beta\left(\epsilon-\tilde \mu\right)}+1}\,d\epsilon\,,
\label{eq:rhoe}\\
\tilde P &= \frac{\gamma^2}{3}\int_1^\infty
\frac{(\sqrt{\epsilon^2-1})^3}{e^{\tilde \beta\left(\epsilon-\tilde \mu\right)}+1}\,d\epsilon\,.
\label{eq:pe}
\end{align}
%
Here we have re-written the integrals in terms of the variable $\epsilon = \sqrt{1+p^2/m^2}$, and we defined the dimensionless coupling $\gamma^2=gGL^2m^4/2\pi^2$.

A convenient re-parametrization of $\lambda$ and $\nu$ in terms of new functions $\tilde{M}$ and $\chi$ is
%
\begin{eqnarray}
&&e^{\lambda}=\left(1-\frac{2 \tilde{M} }{r}+{r^2}\right)^{-1},	
\label{eq:redefinition-lambda}
\\
&&e^{\nu}=e^\chi\left(1-\frac{2 \tilde{M} }{r}+{r^2}\right)\,.
\label{eq:redefinition-nu}
\end{eqnarray}
%
The resulting Einstein equations read
%
\begin{align}
&\frac{d \tilde{M}}{d r}=4\pi\,r^2 \tilde\rho \,,
\label{eq:eqs2a}
\\
%&\frac{d\nu}{d r}=\frac{2}{r^2}\left(M+r^3\left(4\pi\,\tilde P-\frac32%+P_{vac}\right)\right)e^{\lambda(r)}, \\
&\frac{d\chi}{d r}
=8\pi r\left(\tilde P+\tilde\rho\right)e^{\lambda},
%\\
\label{eq:eqs2b}
\end{align}

The equations \eqref{eq:eqs2a}-\eqref{eq:eqs2b}, together with the definitions \eqref{eq:rhoe}-\eqref{eq:pe} in terms of the spatially varying temperature and chemical potentials given by \eqref{eq:tolman3}-\eqref{eq:klein3} must be solved numerically for the variables $\tilde{M}, \chi,\tilde{\rho},\tilde{P}$. Notice that the fermion mass $m$ plays no role other that setting the scale. We choose boundary conditions at the center of the star $r=0$ as
%
\begin{eqnarray}
\tilde{M}(0)&=&0\,,\qquad\qquad\mbox{(or in other words }\lambda(0)=0\mbox{)}\,,\nonumber\\
\chi(0)&=&0\,,\nonumber\\
&&\nonumber\\
\tilde T(0)&=&\tilde T_0\,,\nonumber\\
\tilde \mu(0)&=&\tilde \mu_0\ \equiv\ \Theta_0\Tilde T_0+1\,.
\label{mu0}
\end{eqnarray}
%
Here $\Theta_0$ can be regarded as the central degeneracy. The resulting solutions are indexed by the parameters $\tilde T_0, \Theta_0$ and $\gamma$.
%

\section{The boundary: degenerate fermionic operators at finite temperature}
\label{sec:correlators3}
%

Since the geometry asymptotes to global AdS, its conformal boundary is a cylinder $\mathbb{R}\times S^2$. The $\mathbb{R}$ direction is coordenatized by the variable $t$ on our metric anzatz. Now, in order to put the system in a thermal bath, we have to go to Euclidean time by the Wick rotation $t_E=it$. Then, we compactify the $t_E$ direction in a circle of length $\beta=e^{\frac{\nu-\nu_0}2}\beta_0$ corresponding to the inverse temperature. Since we want the fluid in the bulk to be in equilibrium with the thermal bath, we need to impose $\beta=1/T$ or, by making use of Tolman relation $\beta_0=1/T_0$. On the aforementioned cylinder, the holographic dual is defined as a conformal field theory. Since the Euclidean time direction of the conformal theory is given by $t_E$, its temperature corresponds to $T_0$.

 \begin{tcolorbox}[colback=red!5!white,colframe=red!75!black,title=Hint ...] The geometry that we will use throughout the thesis is global AdS, so its conformal boundary is a cylinder $\mathbb{R}\times S^2$.
\end{tcolorbox}

In order for holography to work, the conformal field theory must have a large central charge. This can be achieved in the present setup without spoiling the perfect fluid approximation, as explained in \cite{deBoer:2009wk}, by taking a proportionally large mass $m$.

In order to probe the above defined background with some conformal field theory observable, we concentrate in the simplest case of a scalar operator.
%
According to the general dictionary of the AdS/CFT correspondence, the Matsubara two point correlator of a boundary scalar operator with large conformal dimension $\Delta\equiv{\sf m} L$, is given as a function of the angular span of the points on the boundary $\Delta\vartheta, \Delta\varphi$ and the elapsed Euclidean time $\Delta t_E$ as
%
\begin{equation}
\langle
{\cal O}(\Delta\vartheta, \Delta\varphi, \Delta t_E){\cal O}(0)
\rangle
=
\lim_{r_\epsilon\to\infty}r_\epsilon^{2{\sf m} L}e^{-S^E_{\sf on-shell}(\Delta\vartheta, \Delta\varphi,\Delta t_E)}\,,
\label{eq:correlator3}
\end{equation}
%
where $r_\epsilon$ is an UV bulk regulator, whose power is included in the prefactor in order to get a finite result. The exponent contains the on-shell form of the Euclidean action for a particle with mass ${\sf m}$ moving in the Euclidean bulk
%
\begin{equation}
S_E ={\sf m} L\int d\tau_E\sqrt{e^{\nu(r)}\, {t'_E}^2+e^{\lambda(r)}\, {r'}^2+r^2({\vartheta'}^2+\sin^2\!\vartheta\,{\varphi'}^2)}\, ,
\label{eq:action-particle}
\end{equation}
%
where $\tau_E$ is the an Euclidean affine parameter and $(~')=\partial_{\tau_E}(~)$. The worldline approximation was used in \cite{Balasubramanian:2011ur} to study thermalization. For details on its implementation see \cite{Giordano:2014kya} and references therein.

Without loss of generality, we can concentrate in trajectories completely contained in the equatorial plane $\vartheta=\pi/2$.
Moreover, this action is invariant under arbitrary reparametrizations of $\tau_E$, which allows us to fix $\tau_E = \varphi$.
%
Restricting to trajectories with constant $t_E$ we end up with
%
\begin{equation}
S_E ={\sf m} L\int d\varphi\sqrt{r^2+e^{\lambda(r)}\,r'^2}\, ,
\label{eq:action-particle-fixed}
\end{equation}
%
The resulting equations for the single dynamical variable $r$ are invariant under $\varphi$ translations, implying the conservation of the quantity
%
\begin{equation}
r_*=\frac{\,r^2}{\sqrt{r^2+e^{\lambda(r)}\,r'^2}}\,.
\label{eq:p-phi}
\end{equation}
%
By evaluating the right hand side at the tip of the trajectory where $r'=0$, we see that $r_*$ corresponds to the radial position of the tip ($r_*(r'=0)=r$) . Solving for $r'$ we get
%
\begin{equation}
r'=\frac r{r_*}e^{-\frac{\lambda(r)}2}\sqrt{r^2-r_*^2}\,.
\label{eq:velocity}
\end{equation}
%
This allows us to relate the integration constant $r_*$ with the angular separation at the boundary $\Delta\varphi$ of the starting and final points of the trajectory
%
\begin{eqnarray}
\Delta \varphi &=&  \int \frac{dr}{r'}
=2r_*\int_{r_*}^{r_\epsilon}\!\!dr \frac{e^{\frac{\lambda(r)}2}}{r\sqrt{r^2-r_*^2}}\,,
\label{eq:anmgular-span}
\end{eqnarray}
%
where we included a cutoff $r_\epsilon$ in the second line, that must be taken to infinity at the end of the calculations.

On the other hand, plugging eq. \eqref{eq:velocity} into the gauge-fixed action  \eqref{eq:action-particle-fixed} results in the on shell form
%
\begin{equation}
S^E_{\sf on-shell}(\Delta\varphi) %=\frac{{\sf m}  L}{r_*}\int\!\!d\varphi r^2
=2{\sf m}  L\int_{r_*}^{r_\epsilon}\!\!dr  \frac{re^{\frac{\lambda(r)}2}}{\sqrt{r^2-r_*^2}}
\label{eq:action-particle-on-shell}
\end{equation}
%
where the same cutoff was included. Notice that, when re-inserted into the correlator \eqref{eq:correlator}, the logarithmic divergence of this integral on the cutoff is canceled by the prefactor, as anticipated.

\section{Results obtained for neutron stars at zero temperature}
\label{sec:results3}

They solved the system (\ref{eq:redefinition-lambda})-(\ref{mu0}) numerically using {\tt Fortran} and {\tt Mathematica} routines, for different values of the parameters $ \tilde T_0, \Theta_0$ and $\gamma$. Some of the density $\tilde{\rho}(r)$ and mass $\tilde{M}(r)$ profiles found in this paper are shown in Figs. \ref{fig:thetaneg} and \ref{fig:thetapos}.

As can be seen in Fig.~\ref{fig:thetapos}, the expected core-halo structure appears at large values central degeneracy $\Theta_0$ and central temperature $\tilde T_0$. In those cases, the density profile $\tilde{\rho}(r)$ presents a central plateau that extends up to a well defined radius $r_c$, identified with the ``core'' of the configuration, and a lower exterior plateau identified with the ``halo''.
Further in $r$, we see that the density drops to zero at a finite radius $r=r_b$, that defines the radius of the star.

The region $r>r_b$ is described by a vacuum Schwarzchild solution with mass $\tilde{M}_b=\tilde{M}(r_b)$, corresponding to the total mass of the star. Similarly to what happens in the asymptotically flat case \cite{Arguelles:2014sfa}, there is a maximum of the mass at a finite critical value of the central density $\tilde{\rho}_{\sf cr}$. Since solutions with higher mass do not exist, this bound is interpreted as the Oppenheimer-Volkoff limit. In the asymptotically flat context, solutions with central densities larger than $\tilde{\rho}_{\sf cr}$ can be shown to be unstable \cite{Schiffrin:2013zta}. We assume that the same is true in the present asymptotically AdS setup.
From the holographic perspective, the gravitational collapse in the bulk can be interpreted as a confinement/deconfinement transition in the dual field theory (analogously to the zero temperature case reported in \cite{Arsiwalla:2011}).

 \begin{tcolorbox}[colback=red!5!white,colframe=red!75!black,title=Hint ...] From the holographic perspective, the gravitational collapse in the bulk can be interpreted as a confinement/deconfinement transition in the dual field theory.
\end{tcolorbox}

%Fig1
\begin{figure}[ht]
	\centering
		\includegraphics[width=1.\textwidth]{Chapters/Thesis2/fig1.png}
	\caption{
		Left: logarithmic plots of the density (up) and mass (down) profiles as functions of the radius, as we approach the critical value of the central temperature (blue curve). Notice that the core and the halo are not well defined for this values of the parameters.
		%
		Right (up): plot of the on-shell actions (which correspond to minus the logarithm of the two-point correlator). Notice the swallow tale structure that appears as we approach the critical value for the central temperature { (to make the structure more evident, we extended the natural rank $(0,\pi)$ of the polar angle $\Delta \varphi$ along the opposite meridian up to $2\pi$)}. A figure taken from the work of \cite{2018JHEP...05..118A}.
		\label{fig:thetaneg}
	}
\end{figure}

%Fig2
\begin{figure}[ht]
	\centering
		\includegraphics[width=1.\textwidth]{Chapters/Thesis2/fig2.png}
	\caption{
		Left: logarithmic plots of the density (up) and mass (down) profiles as functions of the radius, as we approach the critical value of the central temperature (blue curve). Notice the that the core and the halo are well defined for this values of the parameters.
		%
		Right (up): plot of the on-shell actions (which correspond to minus the logarithm of the two-point correlator) as functions of the angle at the boundary. Notice that there is not a swallow tale structure as we approach the critical value for the central temperature { (to compare with the previous figures, we extended the natural rank $(0,\pi)$ of the polar angle $\Delta \varphi$ along the opposite meridian up to $2\pi$)}. A figure taken from the work of \cite{2018JHEP...05..118A}.
		\label{fig:thetapos}
	}
\end{figure}








%Fig6
\begin{figure}[ht]
	\centering
	\begin{subfigure}[b]{\textwidth}
		\includegraphics[width=.46\textwidth]{Chapters/Thesis2/AngleWOSwallowTale.pdf}
		\hfill
		\includegraphics[width=.46\textwidth]{Chapters/Thesis2/CompanionWOSwallowTale.pdf}
	\end{subfigure} 
	\\~\\~\\
	\begin{subfigure}[a]{\textwidth}
		\includegraphics[width=.46\textwidth]{Chapters/Thesis2/AngleSwallowTale.pdf}
		\hfill
		\includegraphics[width=.46\textwidth]{Chapters/Thesis2/CompanionSwallowTale.pdf}
	\end{subfigure}
	\caption{
		Plots of the angular span $\Delta\varphi$ as a function of the apsidal position $r_*$ (left), and the corresponding correlators (right). Top: plots corresponding to the critical temperature  $T=10^{-2}$ at positive central degeneracy $\Theta_0=30$. The angle $\Delta\varphi$ is a monotonic function of $r_*$, resulting in the univalued correlator (the dotted line sits at $\Delta\varphi=3$ intersects the curves only once).
		%
		Bottom: plots corresponding to the critical temperature  $\tilde T=7\times 10^{-2}$ at negative central degeneracy $\Theta_0=-10$. Here the angle oscillates as a function of $r_*$. Since the natural range of the polar angle is $(0,\pi)$, values larger than $\pi$ must be reflected in at $\Delta\varphi=\pi$ (dashed line), resulting in the dashed colored curve. As a result, a given value of the angle corresponds to three values of $r_*$, resulting in a multivalued correlator (the dotted line sits at $\Delta\varphi=3$ intersects the curves three times).
		% 
		\label{fig:angular}}
\end{figure}
%

%Fig7
\begin{figure}[ht]
	\centering
	\qquad\qquad
	\includegraphics[width=.45\textwidth]{Chapters/Thesis2/plot3.pdf}
	\hfill
	\quad
	\includegraphics[width=.35\textwidth]{Chapters/Thesis2/LegendsNeg.pdf}
	\caption{
		Plots of the angular span $\Delta\varphi$ as a function of the apsidal position $r_*$. The plots correspond to the temperatures  depicted in Fig. \ref{fig:thetaneg}, at negative central degeneracy $\Theta_0=-10$. For temperatures $\tilde T \gtrsim 10^{-2}$ the angle $\Delta\varphi$ oscillates as a function of $r_*$, resulting in the multivalued correlator. On the other hand, for  $\tilde T \lesssim 10^{-3}$ the angle $\Delta\varphi$ is monotonic and the correlator is univalued. 
		\label{fig:hump}}
\end{figure}

Another point that is important to understand regarding the boundary study in this paper is the following analysis for the two-point correlators. In the figures they plotted the on-shell action (which correspond to minus its logarithm) { and they extended the natural rank $(0,\pi)$ of the polar angle $\Delta \varphi$ along the opposite meridian up to $2\pi$}. For solutions near to the critical one, they found a ``swallow tale'' structure. This is evident for small central degeneracies $\Theta_0$, and disappears for larger values. One can think that this could be something came from the cut off but they verified that it is not a cutoff effect. This effect is more evident for the more massive configurations, \textit{i.e}. configurations with smaller halos and denser cores (see \emph{e.g.} Figs.~\ref{fig:thetaneg} and \ref{fig:thetapos} for comparison).

 \begin{tcolorbox}[colback=red!5!white,colframe=red!75!black,title=Hint ...] Looking solutions near the critical ones ($T \sim T_c$) they found a ``swallow tale'' structure for the action on shell as a function of the angular separation at the boundary. 
\end{tcolorbox}

\newpage

\section{Discussion}

The most interesting feature found in our solutions in the swallow tale structure present in the correlator. Such ``multivalued'' form for correlators have been reported previously for quenched states in thermalization studies, when the correlator is plotted as a function of the gauge theory time \cite{Balasubramanian:2011ur}- \cite{Giordano:2014kya}. Here, it shows up for near to critical equilibrium states, as a function of the spatial separation. 
When a swallow tale appears in the plots of the free energy as a function of temperature, it is taken as a signal of a phase transition. In our case, such conclusion cannot be drawn without further analysis, that we perform in this section.

From the bulk perspective, the swallow tale structure corresponds to the existence of three different geodesics joining the same points at the boundary.  One of this solutions represents a maximum of the action, the second one represents a saddle point, while the remaining one corresponding to the true minimum. Since the correct value of the dual field theory correlator is given by the curve corresponding to the minimum action, only the lower curve should be kept, and this swallow tale structure corresponds to a discontinuity in the angular derivative of the correlator at antipodal points $\Delta\varphi=\pi$. 

Recall that the angular span $\Delta\varphi$ and the on shell action $S^E_{\sf on~shell}$ are obtained from equations \eqref{eq:anmgular-span} and \eqref{eq:action-particle-on-shell} respectively, as a function of the radial position of the apsidal point of the geodesic $r_*$. Then the curve $S^E_{\sf on~shell}$ {\it vs.} $\Delta\varphi$ is plotted using $r_*$ as an affine parameter. In the cases in which the correlator shows a swallow tale, three values of the on-shell action correspond to the same value of the angle. Since the on-shell action is a well defined function of $r_*$, we conclude that there must be three different values of $r_*$ that return the same value of the angle. In other words, the curve $\Delta\varphi$ versus $r_*$ has an oscillation. 

In order to have an oscillation, the derivative of $\Delta\varphi$ with respect to $r_*$ must change its sign. Rewriting equation \eqref{eq:anmgular-span} in terms of the variable $u=r/r_*$ as
%
\begin{eqnarray}
\Delta \varphi &=&  
2\int_{1}^{\infty}\!\!du \,\frac{e^{\frac{\lambda(r_*u)}2}}{u\sqrt{u^2-1}}\,,
\label{eq:anmgular-span-u}
\end{eqnarray}
%
we can take the derivative with respect to $r_*$, obtaining%\footnote{Here we are assuming that we can interchange differentiation and integration. }
%
%
\begin{eqnarray}
\frac{\partial\Delta\varphi }{\partial r_*} &=&  2
\int_{1}^{\infty}\!\!du \,\frac{\left(e^{\frac{\lambda(r_*u)}2}\right)'}{\sqrt{u^2-1}}\,=
%\nonumber\\
%&=&
2\int_{r_*}^{\infty}\!\!dr \,\frac{e^{\frac{3\lambda(r)}2}}{\sqrt{r^2-r_*^2}}
\left(
\frac{\tilde M'}r-\frac{\tilde M}{r^2}-r
\right)\,,
\label{eq:derivative-anmgular-span-u}
\end{eqnarray}
%
where in the last equality we used \eqref{eq:redefinition-lambda} and reintroduced the variable $r$. This can be rearranged as
%
\begin{eqnarray}
\frac{\partial\Delta\varphi }{\partial r_*} &=&  
2\int_{r_*}^{\infty}\!\!dr \,\frac{e^{\frac{3\lambda(r)}2}}{\sqrt{r^2-r_*^2}}
\,p\,,
\quad\quad\ \quad
{\rm with}
\ \
p=
\left(
\frac{\tilde{M}}{r^2}
\left(\frac{d\log \tilde{M}}{d\log r}-1\right)-r
\right)\,,
\label{eq:derivative-anmgular-span-u-log}
\end{eqnarray}
% 
In order to understand whether the $\Delta \varphi$ oscillates as a function of $r_*$, we need to study whether the above integral changes its sign. The sign of the integrand is fixed by the sign of $p$. The overall sign of the integral for a given value of $r_*$ is then determined by the relative weight of the regions in which $p$ is positive or negative. 

For a radius $r_*$ larger than the radius of the star $r_*>r_b$, the mass function is constant $\tilde{M}=\tilde{M}_b$. Then its logarithmic derivative in $p$ vanishes, resulting in a negative overall value for the integral. This implies ${\partial\Delta\varphi }/{\partial r_*}<0$,  in agreement with the intuition that the further in the interior of the geometry our geodesic reaches, the larger the angular span of the initial and final points in the boundary.

As we move $r_*$ into the halo $r_c<r_*<r_b$, such region starts to contribute to the integral. Since at the halo the density is approximately constant $\tilde{\rho}\simeq\tilde{\rho}_h$ and very small, the mass function takes the  form $\tilde{M}=\tilde{M}_c+{4\pi}\tilde{\rho}_h r^3/3$, that results in $p\simeq 2\tilde{M}_c/r^2-r$.
For light configurations, the first term is small and then $p$ is negative, giving a negative contribution to the integral (this is the case for example for the critical case in Fig. \ref{fig:thetapos}). On the other hand, for dense cores, it results in a positive contribution (as is the case for the critical curve in Fig. \ref{fig:thetaneg}).
Whether such contribution can change the overall sign of the integral to ${\partial\Delta\varphi }/{\partial r_*}>0$ depends on the density of the configuration.

When $r_*$ gets into the core $r_*<r_c$, the mass function can be written as $\tilde{M}=4\pi \tilde{\rho}_c r^3/3$, where $\rho_c$ is the approximately constant core density. We get $p=(8\pi\tilde{\rho}_c-3)r/3$, which is positive for the central densities we considered, resulting in a positive contribution to the integral. Again, such positive contribution may or may not be enough to change the sign of the overall integral, depending of the density of the background.

The conclusion is that a negative derivative ${\partial\Delta\varphi }/{\partial r_*}<0$ is always the case for large $r_*$. On the other hand, for small $r_*$ the derivative still negative for light configurations, but it may become positive if the configuration is massive enough. In order for this to happen, we need that the positive contribution extends for a large enough interval of the radial variable, {\em i.e.} we need an extended core.  
If such is the case, we have an oscilation of $\Delta\varphi$ as a function of $r_*$, that results in a swallow tale in the correlator. See Fig. \ref{fig:angular} for further details. 


As this discussion should make clear, the swallow tale is not a feature of all correlators that grows continuously as we move the parameters, but a distinctive characteristic of dense and extended cores, which is absent in light ones. In other words, the existence or not of a swallow tale sets a frontier on the $(\Theta_0,\tilde T)$ plane, and in such (somewhat limited) sense, it can be regarded as a signal of a phase transition. For example, at negative $\Theta_0=-10$, we see in Fig. \ref{fig:thetaneg} that the transition temperature at which the swallow tale appears is around $T^{-3}\lesssim\tilde T\lesssim 10^{-2}$. In Fig. \ref{fig:hump} we plotted the corresponding $\Delta\varphi$ curves, showing how the oscillation dissapears as the temperature gets smaller. 

%

\newpage
\section{Conclusions}
\label{sec:concusions}
%
We investigated the solution to Einstein equations sourced by to a weakly-coupled self-gravitating fermionic fluid at finite temperature in global AdS spacetime. They form a three-parameter family, indexed by the central degeneracy, the central temperature and the particle mass. According to the value of such parameters, a well defined core-halo structure appears when the mass is large, and it becomes better defined as the central degeneracy grows and the central temperature decreases.

With the obtained backgrounds, we evaluated the two point correlator of a scalar operator of the dual field theory at constant time. We found that it shows a swallow tale structure when evaluated on near to critical solutions with small central degeneracy. This is to be compared to a similar phenomenon previously reported in the case of non-equilibrium quenched states. The presence or absence of such swallow tale sets a frontier in the phase diagram, that allows us to identify separated regions. In such limited sense, the appearance of a swallow tale can be interpreted as a phase transition. 






==> Old/osszefoglalok.tex <==

\chapter*{Összefoglalás}
\markboth{Összefoglalás}{Összefoglalás}
\addcontentsline{toc}{chapter}{Összefoglalás}

Osszefoglalas

A munka három fő témakörből áll. Tomor osszefoglalas.

\section*{1. resz}

1. resz rovid bevezeto.

1. resz ismertetes.

\section*{2. resz}

2. resz rovid bevezeto.

2. resz ismertetes.

\newpage
\section*{3. resz}

3. resz rovid bevezeto.

3. resz ismertetes.
\newpage
\section*{A disszertáció tézisei}

Az \textbf{első téziscsoportban} a hozzájárulásaim az 1. reszhez kapcsolódik. A részletes bemutatás a \ref{chapter_2}. fejezetben található.

\begin{enumerate}[wide = 0pt, widest = {III/5.}, leftmargin =*]
    \item[I/1.] Hozzajarulas I.
    
    \item[I/2.] Hozzajarulas II.

    \item[I/3.] Hozzajarulas III.
    
    \item[I/4.] Hozzajarulas IV.
\end{enumerate}

\noindent
A \textbf{második téziscsoport} 2. részhez kapcsolódik. A részletes bemutatás a \ref{chapter_3}. fejezetben található.

\begin{enumerate}[wide = 0pt, widest = {III/5.}, leftmargin =*]
    \item[II/1.] Hozzajarulas I.
    
    \item[II/2.] Hozzajarulas II.

    \item[II/3.] Hozzajarulas III.
    
    \item[II/4.] Hozzajarulas IV.
\end{enumerate}

\noindent
A \textbf{harmadik téziscsoport} hozzájárulásai a 3. részhez kapcsolódnak. Részletes bemutatás a \ref{chapter_4}. fejezetben található.

\begin{enumerate}[wide = 0pt, widest = {III/5.}, leftmargin =*]
       \item[III/1.] Hozzajarulas I.
    
    \item[III/2.] Hozzajarulas II.

    \item[III/3.] Hozzajarulas III.
    
    \item[III/4.] Hozzajarulas IV.
\end{enumerate}
